Applications of Psychological Science for Actionable Analytics

Actionable analytics are those that humans can understand, and operationalize. What kind of data mining models generate such actionable analytics? According to psychological scientists, humans understand models that most match their own internal models, which they characterize as lists of "heuristic" (i.e., lists of very succinct rules). One such heuristic rule generator is the Fast-and-Frugal Trees (FFT) preferred by psychological scientists. Despite their successful use in many applied domains, FFTs have not been applied in software analytics. Accordingly, this paper assesses FFTs for software analytics. We find that FFTs are remarkably effective. Their models are very succinct (5 lines or less describing a binary decision tree). These succinct models outperform state-of-the-art defect prediction algorithms defined by Ghortra et al. at ICSE'15. Also, when we restrict training data to operational attributes (i.e., those attributes that are frequently changed by developers), FFTs perform much better than standard learners. Our conclusions are two-fold. Firstly, there is much that software analytics community could learn from psychological science. Secondly, proponents of complex methods should always baseline those methods against simpler alternatives. For example, FFTs could be used as a standard baseline learner against which other software analytics tools are compared.

==> fft_fse18 (1)/change_freq.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=.8\linewidth]{img/change_freq.png}
    \caption{Only some metrics
      change between
      versions $i$ and $i+1$ of a software system.
      For definitions of the metrics
      on the x-axis, see \tabl{metrics}.
      To create this plot, we
      studied the  26  versions
      of the ten datasets
      in \tabl{data}.
      First we initialize $total=0$, then for all pairs of versions $i,i+1$ from the same data set,  we 
        (a)~incremented $\mathit{total}$ by one;
(b)~collected  the  distributions of metric $m$
seen in version $i$ and $i+1$ of the software;
(c)~ checked if  those two distributions were different;
and if so, (d)~added one to  $\mathit{changed_m}$.
Afterwards, the y-axis of this plot was
  computed using $100*\mathit{changed_m}/\mathit{total}$.}
    \label{fig:change_freq}
\end{figure}

==> fft_fse18 (1)/data.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!b]
\centering
\scriptsize
\caption{Some open-source JAVA systems. Used for training and testing showing different details for each. 
All   data   available on-line at http://tiny.cc/seacraft. }
\label{tab:data}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
         & \multicolumn{2}{l|}{\cellcolor[HTML]{C0C0C0}Training} & \multicolumn{3}{l|}{\cellcolor[HTML]{C0C0C0}Testing} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Data Set & Versions                         & Cases              & Versions        & Cases        & \% Defective        \\ \hline
jedit    & 3.2, 4.0, 4.1, 4.2               & 1257               & 4.3             & 492          & 2                   \\ \hline
ivy      & 1.1, 1.4                         & 352                & 2.0             & 352          & 11                  \\ \hline
camel    & 1.0, 1.2, 1.4                    & 1819               & 1.6             & 965          & 19                  \\ \hline
synapse  & 1.0, 1.1                         & 379                & 1.2             & 256          & 34                  \\ \hline
velocity & 1.4, 1.5                         & 410                & 1.6             & 229          & 34                  \\ \hline
lucene   & 2.0, 2.2                         & 442                & 2.4             & 340          & 59                  \\ \hline
poi      & 1.5, 2, 2.5                      & 936                & 3.0             & 442          & 64                  \\ \hline
xerces   & 1.0, 1.2, 1.3                    & 1055               & 1.4             & 588          & 74                  \\ \hline
log4j    & 1.0, 1.1                         & 244                & 1.2             & 205          & 92                  \\ \hline
xalan    & 2.4, 2.5, 2.6                    & 2411               & 2.7             & 909          & 99                  \\ \hline
\end{tabular}
}
\end{table}

==> fft_fse18 (1)/frequencies.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}
  \centering
  
  \footnotesize
  \caption{ Frequency heatmap of best exit polices seen for  FFT and defect prediction.}\label{tab:xcept}
  \vspace{5mm}
  \resizebox{\columnwidth}{!}{%
  \label{tab:fft-frequency}%
    \begin{tabular}{c|r|r|r|r|r}
    \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{l|}{Best FFF} &       & \multicolumn{2}{c|}{\textbf{25\%  }} & \multicolumn{2}{c}{\textbf{100\%  }} \\
    
    \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{5em}|}{\textbf{exit policy}} &       & \multicolumn{1}{p{2.25em}|}{D2H} & \multicolumn{1}{p{2.25em}|}{$P_{\mathit{opt}}$ } & \multicolumn{1}{p{2.25em}|}{D2H} & \multicolumn{1}{p{2.25em}}{$P_{\mathit{opt}}$} \\
    
    % \rowcolor[rgb]{ .851,  .851,  .851} \multicolumn{1}{p{5em}|}{\textbf{exit policy}} & \multicolumn{1}{p{2.25em}|}{\textbf{Sum}} & \multicolumn{1}{p{2.25em}|}{\textbf{D2H}} & \multicolumn{1}{p{2.25em}|}{$P_{\mathit{opt}}$} & \multicolumn{1}{p{2.25em}|}{\textbf{D2H}} & \multicolumn{1}{p{2.25em}}{$P_{\mathit{opt}}$} \\
    
    \rowcolor[rgb]{ .988,  .988,  1} 00001 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 00010 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 00101 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 00110 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 01001 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 01010 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 01101 & \cellcolor[rgb]{ .988,  .949,  .961}1 & 0     & 0     & 0     & \cellcolor[rgb]{ .988,  .949,  .961}1 \\
    \rowcolor[rgb]{ .988,  .988,  1} 01110 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 10001 & \cellcolor[rgb]{ .973,  .412,  .42}14 & \cellcolor[rgb]{ .984,  .741,  .753}6 & 0     & \cellcolor[rgb]{ .98,  .702,  .71}7 & \cellcolor[rgb]{ .988,  .949,  .961}1 \\
    \rowcolor[rgb]{ .988,  .988,  1} 10010 & \cellcolor[rgb]{ .980,  .659,  .671}8 & \cellcolor[rgb]{ .984,  .824,  .835}4 & \cellcolor[rgb]{ .988,  .906,  .918}2 & \cellcolor[rgb]{ .988,  .906,  .918}2     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 10101 & \cellcolor[rgb]{ .988,  .867,  .878}3 & 0     & \cellcolor[rgb]{ .988,  .949,  .961}1 & \cellcolor[rgb]{ .988,  .949,  .961}1 & \cellcolor[rgb]{ .988,  .949,  .961}1 \\
    \rowcolor[rgb]{ .988,  .988,  1} 10110 & \cellcolor[rgb]{ .984,  .784,  .796}5 & 0     & \cellcolor[rgb]{ .988,  .867,  .878}3 & 0     & \cellcolor[rgb]{ .988,  .906,  .918}2 \\
    \rowcolor[rgb]{ .988,  .988,  1} 11001 & 0     & 0     & 0     & 0     & 0 \\
    \rowcolor[rgb]{ .988,  .988,  1} 11010 & \cellcolor[rgb]{ .988,  .867,  .878}3 & 0     & \cellcolor[rgb]{ .988,  .949,  .961}1 & 0     & \cellcolor[rgb]{ .988,  .906,  .918}2 \\
    \rowcolor[rgb]{ .988,  .988,  1} 11101 & \cellcolor[rgb]{ .988,  .906,  .918}2 & 0     & 0     & 0     & \cellcolor[rgb]{ .988,  .906,  .918}2 \\
    \rowcolor[rgb]{ .988,  .988,  1} 11110 & \cellcolor[rgb]{ .984,  .824,  .835}4 & 0     & \cellcolor[rgb]{ .988,  .867,  .878}3 & 0     & \cellcolor[rgb]{ .988,  .949,  .961}1 \\\hline
   Totals &  40 & 10 & 10 & 10 & 10 
    \end{tabular}%
    }
    \vspace{5mm}
\end{table}%


==> fft_fse18 (1)/issue_lifetime.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}
\centering
\caption{Which learners performed better (in terms of   median {\em Dis2heaven}) in  5*10 cross-value experiments predicting
for different classes of ``how long to close an Github issue''.
Gray areas denote experiments where FFTs were out-performed by other learners.  Note that, in (43/56=77\%) experiments, FFT performed better
than the prior state-of-the-art in this area~\cite{rahul2018bellwhether}.}
\label{tab:issue_lifetime}
\resizebox{0.45\textwidth}{!}{%
\begin{threeparttable}
% \begin{tabular}{l|l|l|l|l|l|l|l|}
%                                 & \multicolumn{7}{c|}{\textbf{Days till closed}}                                                                                                                                               \\ \cline{2-8} 
% \textbf{Data(\# of instances)} & \textbf{$>365$ }            & \textbf{$<180$  }            & \textbf{$<90$  }                      & \textbf{$<30$  } & \textbf{$<14$  } & \textbf{$<7$  }              & \textbf{$<1$  }               \\ \hline
% cloudstack (1551)               & 2\%                          & 4\%                          & 9\%                                   & 7\%              & 7\%              & \cellcolor[HTML]{C0C0C0}29\% & \cellcolor[HTML]{C0C0C0}42\% \\
% node (6207)                     & 3\%                          & 4\%                          & 9\%                                   & 7\%              & 8\%              & \cellcolor[HTML]{C0C0C0}29\% & \cellcolor[HTML]{C0C0C0}39\% \\
% deeplearning (1434)             & 2\%                          & 3\%                          & 5\%                                   & 5\%              & 5\%              & 15\%                         & \cellcolor[HTML]{C0C0C0}65\% \\
% cocoon (2045)                   & 4\%                          & 3\%                          & 4\%                                   & 2\%              & 2\%              & 4\%                          & 6\%                          \\
% ofbiz (6177)                    & 6\%                          & 8\%                          & 9\%                                   & 8\%              & 8\%              & 19\%                         & 25\%                         \\
% camel (5056)                    & \cellcolor[HTML]{C0C0C0}41\% & \cellcolor[HTML]{C0C0C0}13\% & \cellcolor[HTML]{FFFFFF}6\%           & 3\%              & 3\%              & 9\%                          & 14\%                         \\
% hadoop (12191)                  & \cellcolor[HTML]{C0C0C0}18\% & \cellcolor[HTML]{C0C0C0}18\% & \cellcolor[HTML]{C0C0C0}\textit{14\%} & 3\%              & 1\%              & 1\%                          & 0\%                          \\
% qpid (5475)                     & \cellcolor[HTML]{C0C0C0}10\% & \cellcolor[HTML]{C0C0C0}16\% & \cellcolor[HTML]{C0C0C0}10\%          & 3\%              & 2\%              & 3\%                          & 4\%                         
% \end{tabular}
\begin{tabular}{|l|l|l|l|l|l|l|l|}
\hline
                                & \multicolumn{7}{c|}{\textbf{Days till closed}}                                                                                                                                                                 \\ \cline{2-8} 
\textbf{Data(\# of instances)} & \textbf{$>365$ }            & \textbf{$<180$  }            & \textbf{$<90$  }                      & \textbf{$<30$  } & \textbf{$<14$  } & \textbf{$<7$  }              & \textbf{$<1$  }               \\ \hline
cloudstack (1551)               & FFT                            & FFT                           & FFT                                 & FFT                   & FFT                   & \cellcolor[HTML]{C0C0C0}DT & \cellcolor[HTML]{C0C0C0}LR \\ \hline
node (6207)                     & FFT                            & FFT                           & FFT                                 & FFT                   & FFT                   & \cellcolor[HTML]{C0C0C0}DT & \cellcolor[HTML]{C0C0C0}LR \\ \hline
deeplearning (1434)             & FFT                            & FFT                           & FFT                                 & FFT                   & FFT                   & FFT                        & \cellcolor[HTML]{C0C0C0}RF \\ \hline
cocoon (2045)                   & FFT                            & FFT                           & FFT                                 & FFT                   & FFT                   & FFT                        & FFT                        \\ \hline
ofbiz (6177)                    & FFT                            & FFT                           & FFT                                 & FFT                   & FFT                   & FFT                        & FFT                        \\ \hline
camel (5056)                    & \cellcolor[HTML]{C0C0C0}RF/KNN & \cellcolor[HTML]{C0C0C0}KNN   & \cellcolor[HTML]{FFFFFF}FFT/KNN/DT  & FFT                   & FFT                   & FFT                        & FFT                        \\ \hline
hadoop (12191)                  & \cellcolor[HTML]{C0C0C0}KNN    & \cellcolor[HTML]{C0C0C0}DT    & \cellcolor[HTML]{C0C0C0}\textit{DT} & FFT                   & FFT                   & FFT                        & FFT                        \\ \hline
qpid (5475)                     & \cellcolor[HTML]{C0C0C0}DT     & \cellcolor[HTML]{C0C0C0}DT/RF & \cellcolor[HTML]{C0C0C0}DT          & FFT                   & FFT                   & FFT                        & FFT                        \\ \hline
\end{tabular}
\begin{tablenotes}
    \item The goal here is to classify an issue according to how long it will
take to close; i.e. less than  1 day, less than 7 days, and so on. 
Values collected via a 5x10 cross-validation procedure.   
   \item Cells with a (white, gray) background means FFTs are statistically (better, worse) than (all, any) of the state-of-the-art learners (as determined  by a Mann-Whitney test, 95\% confidence), respectively. KNN, DT, RF and LR represents K-Nearest Neighbors, Decision Tree, Random Forest and Logistic Regression respectively.
\end{tablenotes}
\end{threeparttable}
}
\end{table}

==> fft_fse18 (1)/issue_lifetime_metrics.tex <==
\begin{table}[!t]
\centering
\caption{Metrics used in issue lifetimes data}
\label{tab:issue_lifetime_metrics}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lll}
\textbf{Commit}                              & \textbf{Comment}                      & \textbf{Issue}                \\ \hline
\multicolumn{1}{l|}{nCommitsByActorsT}       & \multicolumn{1}{l|}{meanCommentSizeT} & issueCleanedBodyLen           \\
\multicolumn{1}{l|}{nCommitsByCreator}       & \multicolumn{1}{l|}{nComments}        & nIssuesByCreator              \\
\multicolumn{1}{l|}{nCommitsByUniqueActorsT} & \multicolumn{1}{l|}{}                 & nIssuesByCreatorClosed        \\
\multicolumn{1}{l|}{nCommitsInProject}       & \multicolumn{1}{l|}{}                 & nIssuesCreatedInProject       \\
\multicolumn{1}{l|}{nCommitsProjectT}        & \multicolumn{1}{l|}{}                 & nIssuesCreatedInProjectClosed \\
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                 & nIssuesCreatedProjectClosedT  \\
\multicolumn{1}{l|}{}                        & \multicolumn{1}{l|}{}                 & nIssuesCreatedProjectT        \\ \hline
\multicolumn{1}{l|}{Misc.}                   & \multicolumn{2}{l}{nActors, nLabels, nSubscribedByT}                 \\ \hline
\end{tabular}
}
\end{table}

==> fft_fse18 (1)/learners.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[!t]
\centering
\small
\caption{For the purposes of predicting
software defects, Ghotra et al.~\cite{ghotra2015revisiting} found that many learners
have similar performance. Here are their four clusters of 32 data mining algorithms.
For our work, we selected learners  at random, one  from each cluster (see the \underline{\textbf{underlined}}
entries). }
\label{tab:learners}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
\begin{tabular}[c]{@{}l@{}}Overall \\ Rank\end{tabular} & \begin{tabular}[c]{@{}l@{}}Classification \\ Technique\end{tabular}                                                               & \begin{tabular}[c]{@{}l@{}}Median \\ Rank\end{tabular} & \begin{tabular}[c]{@{}l@{}}Average \\ Rank\end{tabular} & \begin{tabular}[c]{@{}l@{}}Standard \\ Deviation\end{tabular} \\ \hline
1                                                       & \begin{tabular}[c]{@{}l@{}}Rsub+J48, \underline{\textbf{SL}}, Rsub+SL, \\ Bag+SL, LMT, RF+SL, \\ RF+J48, Bag+LMT, \\ Rsub+LMT, and RF+LMT\end{tabular} & 1.7                                                    & 1.63                                                    & 0.33                                                          \\ \hline
2                                                       & \begin{tabular}[c]{@{}l@{}}RBFs, Bag+J48, Ad+SL, \\ KNN, RF+NB, Ad+LMT, \\ \underline{\textbf{NB}}, Rsub+NB, and Bag+NB\end{tabular}                   & 2.8                                                    & 2.84                                                    & 0.41                                                          \\ \hline
3                                                       & \begin{tabular}[c]{@{}l@{}}Ripper, \underline{\textbf{EM}}, J48, Ad+NB, \\ Bag+SMO, Ad+J48, \\ Ad+SMO, and K-means\end{tabular}                        & 5.1                                                    & 5.13                                                    & 0.46                                                          \\ \hline
4                                                       & \begin{tabular}[c]{@{}l@{}}RF+SMO, Ridor, \underline{\textbf{SMO}}, \\ and Rsub+SMO\end{tabular}                                                       & 6.5                                                    & 6.45                                                    & 0.25                                                          \\ \hline
\end{tabular}
}
\end{table}

==> fft_fse18 (1)/metrics.tex <==
\begin{table*}
\scriptsize
    \renewcommand{\baselinestretch}{0.7}
    
    \caption{The C-K OO metrics studied in \fig{change_freq}. Note that the last line. \textit{`defect'}, denotes the dependent variable.}\label{tab:metrics}
    \begin{center}
    {
    \begin{tabular}{l|l|p{4.0in}}
    \rowcolor{lightgray}
    \hline
    Metric & Name & Description \\ \hline
    amc & average method complexity & Number of JAVA byte codes\\\hline
    avg\_cc & average McCabe & Average McCabe's cyclomatic complexity seen
    in class\\\hline
    ca & afferent couplings & How many other classes use the specific
    class. \\\hline
    cam & cohesion amongst classes & Summation of number of different
    types of method parameters in every method divided by a multiplication
    of number of different method parameter types in whole class and
    number of methods. \\\hline
    cbm &coupling between methods &  Total number of new/redefined methods
    to which all the inherited methods are coupled\\\hline
    cbo & coupling between objects & Increased when the methods of one
    class access services of another.\\\hline
    ce & efferent couplings & How many other classes is used by the
    specific class. \\\hline
    dam & data access & Ratio of  private (protected)
    attributes to   total   attributes\\\hline
    dit & depth of inheritance tree &  It's defined as the maximum length from the node to the root of the tree\\\hline
    ic & inheritance coupling &  Number of parent classes to which a given
    class is coupled (includes counts of methods and variables inherited)
    \\\hline
    lcom & lack of cohesion in methods &Number of pairs of methods that do
    not share a reference to an instance variable.\\\hline
    locm3 & another lack of cohesion measure & If $m,a$ are  the number of
    $methods,attributes$
    in a class number and $\mu(a)$  is the number of methods accessing an
    attribute, 
    then
    $lcom3=((\frac{1}{a} \sum_j^a \mu(a_j)) - m)/ (1-m)$.
    \\\hline
    loc & lines of code & Total lines of code in this file or package.\\\hline
    max\_cc & Maximum McCabe & maximum McCabe's cyclomatic complexity seen
    in class\\\hline
    mfa & functional abstraction & Number of methods inherited by a class
    plus number of methods accessible by member methods of the
    class\\\hline
    moa &  aggregation &  Count of the number of data declarations (class
    fields) whose types are user defined classes\\\hline
    noc &  number of children & Number of direct descendants (subclasses) for each class\\\hline
    npm & number of public methods & npm metric simply counts all the methods in a class that are declared as public. \\\hline
    rfc & response for a class &Number of  methods invoked in response to
    a message to the object.\\\hline
    wmc & weighted methods per class & A class with more member functions than its peers is considered to be more complex and therefore more error prone \\\hline
    
    defect & defect & Boolean: where defects found in post-release bug-tracking systems. \\\hline
    \end{tabular}
    }
    \end{center}
    
\end{table*}

==> fft_fse18 (1)/p_opt_performances.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{\columnwidth}{!}{%
        \begin{tabular}{lrrrrrrr}
\cmidrule{1-1}          & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
D2H} & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
LOC} & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
ACC} & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}SL  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}NB  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}EM  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}SMO  } \\
    \rowcolor[rgb]{ .725,  .725,  .725} camel & \cellcolor[rgb]{ 1,  .918,  .518}.36 & \cellcolor[rgb]{ .996,  .784,  .494}.53 & \cellcolor[rgb]{ .992,  .776,  .49}.54 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .663,  .824,  .498}.17 & \cellcolor[rgb]{ .651,  .82,  .494}.16 & \cellcolor[rgb]{ .996,  .839,  .502}.46 \\
    \rowcolor[rgb]{ .725,  .725,  .725} ivy   & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .565,  .792,  .49}.12 & \cellcolor[rgb]{ .514,  .78,  .486}.09 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .753,  .847,  .502}.22 \\
    \rowcolor[rgb]{ .725,  .725,  .725} jedit & \cellcolor[rgb]{ .412,  .749,  .482}.04 & \cellcolor[rgb]{ 1,  .894,  .514}.39 & \cellcolor[rgb]{ 1,  .894,  .514}.39 & \cellcolor[rgb]{ .541,  .788,  .49}.11 & \cellcolor[rgb]{ .529,  .784,  .49}.10 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .761,  .851,  .502}.22 \\
    \rowcolor[rgb]{ .725,  .725,  .725} log4j & \cellcolor[rgb]{ .996,  .918,  .514}.35 & \cellcolor[rgb]{ .992,  .757,  .486}.56 & \cellcolor[rgb]{ .976,  .424,  .424}.99 & \cellcolor[rgb]{ .702,  .835,  .498}.19 & \cellcolor[rgb]{ .765,  .851,  .502}.22 & \cellcolor[rgb]{ .659,  .824,  .498}.17 & \cellcolor[rgb]{ .871,  .882,  .51}.28 \\
    \rowcolor[rgb]{ .725,  .725,  .725} lucene & \cellcolor[rgb]{ 1,  .922,  .518}.35 & \cellcolor[rgb]{ .984,  .561,  .451}.81 & \cellcolor[rgb]{ .988,  .667,  .471}.68 & \cellcolor[rgb]{ 1,  .863,  .51}.42 & \cellcolor[rgb]{ .875,  .882,  .51}.28 & \cellcolor[rgb]{ .714,  .839,  .498}.20 & \cellcolor[rgb]{ .553,  .792,  .49}.11 \\
    \rowcolor[rgb]{ .725,  .725,  .725} poi   & \cellcolor[rgb]{ .996,  .788,  .494}.52 & \cellcolor[rgb]{ .984,  .604,  .459}.76 & \cellcolor[rgb]{ .984,  .616,  .459}.74 & \cellcolor[rgb]{ .992,  .761,  .486}.56 & \cellcolor[rgb]{ .671,  .824,  .498}.17 & \cellcolor[rgb]{ .953,  .906,  .514}.33 & \cellcolor[rgb]{ .988,  .686,  .475}.65 \\
    \rowcolor[rgb]{ .725,  .725,  .725} synapse & \cellcolor[rgb]{ .988,  .918,  .514}.34 & \cellcolor[rgb]{ 1,  .859,  .506}.43 & \cellcolor[rgb]{ .996,  .824,  .502}.48 & \cellcolor[rgb]{ .78,  .859,  .502}.23 & \cellcolor[rgb]{ .8,  .863,  .506}.24 & \cellcolor[rgb]{ .761,  .851,  .502}.22 & \cellcolor[rgb]{ .996,  .824,  .502}.48 \\
    \rowcolor[rgb]{ .725,  .725,  .725} velocity & \cellcolor[rgb]{ 1,  .886,  .514}.40 & \cellcolor[rgb]{ .988,  .698,  .475}.64 & \cellcolor[rgb]{ 1,  .914,  .518}.36 & \cellcolor[rgb]{ .988,  .69,  .475}.65 & \cellcolor[rgb]{ .988,  .647,  .467}.70 & \cellcolor[rgb]{ .796,  .863,  .506}.24 & \cellcolor[rgb]{ .988,  .678,  .475}.66 \\
    \rowcolor[rgb]{ .725,  .725,  .725} xalan & \cellcolor[rgb]{ .996,  .839,  .502}.46 & \cellcolor[rgb]{ .976,  .42,  .424}.99 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 & \cellcolor[rgb]{ .557,  .792,  .49}.11 & \cellcolor[rgb]{ .627,  .812,  .494}.15 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 \\
    \rowcolor[rgb]{ .725,  .725,  .725} xerces & \cellcolor[rgb]{ .996,  .804,  .498}.50 & \cellcolor[rgb]{ .976,  .459,  .431}.94 & \cellcolor[rgb]{ .976,  .459,  .431}.94 & \cellcolor[rgb]{ .388,  .745,  .482}.02 & \cellcolor[rgb]{ .537,  .784,  .49}.10 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .98,  .525,  .443}.86 \\
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> fft_fse18 (1)/top_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\centering
\caption{Top 25\% features for each PROMISE dataset}
\label{tab:top_features}
{\small
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
Data     & No.1 & No.2 & No.3    & No.4    & No.5    \\ \hline
camel    & amc  & loc  & avg\_cc & mfa     & lcom    \\ \hline
ivy      & loc  & amc  & avg\_cc & lcom    & rfc     \\ \hline
jedit    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
log4j    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
lucene   & amc  & loc  & avg\_cc & cam     & mfa     \\ \hline
poi      & amc  & loc  & lcom    & cam     & avg\_cc \\ \hline
synapse  & loc  & amc  & avg\_cc & lcom    & rfc     \\ \hline
velocity & amc  & loc  & mfa     & avg\_cc & lcom    \\ \hline
xalan    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
xerces   & amc  & loc  & avg\_cc & rfc     & lcom    \\ \hline
\end{tabular}
}
\end{table}


==> p_opt_performances.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
  \resizebox{\columnwidth}{!}{%
        \begin{tabular}{lrrrrrrr}
\cmidrule{1-1}          & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
D2H} & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
LOC} & \multicolumn{1}{p{3.585em}}{\cellcolor[rgb]{ .725,  .725,  .725}FFT-
ACC} & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}SL  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}NB  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}EM  } & \multicolumn{1}{l}{\cellcolor[rgb]{ .725,  .725,  .725}SMO  } \\
    \rowcolor[rgb]{ .725,  .725,  .725} camel & \cellcolor[rgb]{ 1,  .918,  .518}.36 & \cellcolor[rgb]{ .996,  .784,  .494}.53 & \cellcolor[rgb]{ .992,  .776,  .49}.54 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .663,  .824,  .498}.17 & \cellcolor[rgb]{ .651,  .82,  .494}.16 & \cellcolor[rgb]{ .996,  .839,  .502}.46 \\
    \rowcolor[rgb]{ .725,  .725,  .725} ivy   & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .565,  .792,  .49}.12 & \cellcolor[rgb]{ .514,  .78,  .486}.09 & \cellcolor[rgb]{ .863,  .882,  .51}.28 & \cellcolor[rgb]{ .753,  .847,  .502}.22 \\
    \rowcolor[rgb]{ .725,  .725,  .725} jedit & \cellcolor[rgb]{ .412,  .749,  .482}.04 & \cellcolor[rgb]{ 1,  .894,  .514}.39 & \cellcolor[rgb]{ 1,  .894,  .514}.39 & \cellcolor[rgb]{ .541,  .788,  .49}.11 & \cellcolor[rgb]{ .529,  .784,  .49}.10 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .761,  .851,  .502}.22 \\
    \rowcolor[rgb]{ .725,  .725,  .725} log4j & \cellcolor[rgb]{ .996,  .918,  .514}.35 & \cellcolor[rgb]{ .992,  .757,  .486}.56 & \cellcolor[rgb]{ .976,  .424,  .424}.99 & \cellcolor[rgb]{ .702,  .835,  .498}.19 & \cellcolor[rgb]{ .765,  .851,  .502}.22 & \cellcolor[rgb]{ .659,  .824,  .498}.17 & \cellcolor[rgb]{ .871,  .882,  .51}.28 \\
    \rowcolor[rgb]{ .725,  .725,  .725} lucene & \cellcolor[rgb]{ 1,  .922,  .518}.35 & \cellcolor[rgb]{ .984,  .561,  .451}.81 & \cellcolor[rgb]{ .988,  .667,  .471}.68 & \cellcolor[rgb]{ 1,  .863,  .51}.42 & \cellcolor[rgb]{ .875,  .882,  .51}.28 & \cellcolor[rgb]{ .714,  .839,  .498}.20 & \cellcolor[rgb]{ .553,  .792,  .49}.11 \\
    \rowcolor[rgb]{ .725,  .725,  .725} poi   & \cellcolor[rgb]{ .996,  .788,  .494}.52 & \cellcolor[rgb]{ .984,  .604,  .459}.76 & \cellcolor[rgb]{ .984,  .616,  .459}.74 & \cellcolor[rgb]{ .992,  .761,  .486}.56 & \cellcolor[rgb]{ .671,  .824,  .498}.17 & \cellcolor[rgb]{ .953,  .906,  .514}.33 & \cellcolor[rgb]{ .988,  .686,  .475}.65 \\
    \rowcolor[rgb]{ .725,  .725,  .725} synapse & \cellcolor[rgb]{ .988,  .918,  .514}.34 & \cellcolor[rgb]{ 1,  .859,  .506}.43 & \cellcolor[rgb]{ .996,  .824,  .502}.48 & \cellcolor[rgb]{ .78,  .859,  .502}.23 & \cellcolor[rgb]{ .8,  .863,  .506}.24 & \cellcolor[rgb]{ .761,  .851,  .502}.22 & \cellcolor[rgb]{ .996,  .824,  .502}.48 \\
    \rowcolor[rgb]{ .725,  .725,  .725} velocity & \cellcolor[rgb]{ 1,  .886,  .514}.40 & \cellcolor[rgb]{ .988,  .698,  .475}.64 & \cellcolor[rgb]{ 1,  .914,  .518}.36 & \cellcolor[rgb]{ .988,  .69,  .475}.65 & \cellcolor[rgb]{ .988,  .647,  .467}.70 & \cellcolor[rgb]{ .796,  .863,  .506}.24 & \cellcolor[rgb]{ .988,  .678,  .475}.66 \\
    \rowcolor[rgb]{ .725,  .725,  .725} xalan & \cellcolor[rgb]{ .996,  .839,  .502}.46 & \cellcolor[rgb]{ .976,  .42,  .424}.99 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 & \cellcolor[rgb]{ .557,  .792,  .49}.11 & \cellcolor[rgb]{ .627,  .812,  .494}.15 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 & \cellcolor[rgb]{ .973,  .412,  .42}1.00 \\
    \rowcolor[rgb]{ .725,  .725,  .725} xerces & \cellcolor[rgb]{ .996,  .804,  .498}.50 & \cellcolor[rgb]{ .976,  .459,  .431}.94 & \cellcolor[rgb]{ .976,  .459,  .431}.94 & \cellcolor[rgb]{ .388,  .745,  .482}.02 & \cellcolor[rgb]{ .537,  .784,  .49}.10 & \cellcolor[rgb]{ .639,  .816,  .494}.16 & \cellcolor[rgb]{ .98,  .525,  .443}.86 \\
    \end{tabular}%
    }
  \label{tab:addlabel}%
\end{table}%


==> top_features.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[t!]
\centering
\caption{Top 25\% features for each PROMISE dataset}
\label{tab:top_features}
{\small
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|}
\hline
\rowcolor[HTML]{C0C0C0} 
Data     & No.1 & No.2 & No.3    & No.4    & No.5    \\ \hline
camel    & amc  & loc  & avg\_cc & mfa     & lcom    \\ \hline
ivy      & loc  & amc  & avg\_cc & lcom    & rfc     \\ \hline
jedit    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
log4j    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
lucene   & amc  & loc  & avg\_cc & cam     & mfa     \\ \hline
poi      & amc  & loc  & lcom    & cam     & avg\_cc \\ \hline
synapse  & loc  & amc  & avg\_cc & lcom    & rfc     \\ \hline
velocity & amc  & loc  & mfa     & avg\_cc & lcom    \\ \hline
xalan    & amc  & loc  & avg\_cc & lcom    & rfc     \\ \hline
xerces   & amc  & loc  & avg\_cc & rfc     & lcom    \\ \hline
\end{tabular}
}
\end{table}

